Pushing the Limits of In-Network Caching for Key-Value Stores

We present OrbitCache, a new in-network caching architecture that can cache variable-length items to balance a wide range of key-value workloads. Unlike existing works, OrbitCache does not cache hot items in the switch memory. Instead, we make hot items revisit the switch data plane continuously by exploiting packet recirculation. Our approach keeps cached key-value pairs in the switch data plane while freeing them from item size limitations caused by hardware constraints. We implement an OrbitCache prototype on an Intel Tofino switch. Our experimental results show that OrbitCache can balance highly skewed workloads and is robust to various system conditions.

==> sections/ack.tex <==
\section*{Acknowledgement}


==> sections/overview.tex <==
\section{\sys Architecture \label{overview}}
\begin{figure}[t!]
\centering
\includegraphics[width=8.0cm]{./figures/overview.eps}
\caption{\sys architecture. \label{fig:overview}}
\end{figure}

\sys provides high performance, high availability, and strong consistency for replicated systems when handling group membership update events.
This is achieved by an in-network group membership manager that is located on the path between the clients and storage servers, as shown in Figure~\ref{fig:overview}.
Since modern cloud services generally co-locate the servers of a replication group in the same storage rack, our approach is implemented on the ToR switch.
A replication group is either a replicated shard of a rack-scale distributed data store or a replicated coordination service.

\begin{figure}[t!]
\centering
\includegraphics[width=8.0cm]{./figures/header.eps}
\caption{\sys packet format. \label{fig:header}}
\end{figure}

